Learning to Adapt and Calibrate: Score Distribution Alignment for Few-Shot Uncertainty Prediction in Medical VLMs

Uncertainty estimation for medical vision--language models (VLMs) using conformal prediction has gained increasing attention due to its distribution-free coverage guarantees. However, standard conformal prediction relies on exchangeability between calibration and test data and typically requires a sufficiently large calibration set to obtain reliable coverage. These assumptions are difficult to satisfy in few-shot transfer settings, where only a small labeled support set is available to adapt a pretrained VLM to a new medical task, while an unlabeled query set is used for evaluation. Supervised fine-tuning on the support set changes the model parameters and consequently shifts the nonconformity score distribution, breaking exchangeability between calibration and query samples and leading to unreliable coverage under distribution shift. Existing transductive conformal adaptation methods often preserve validity by avoiding supervised updates. While this helps maintain conformal assumptions, it underutilizes the scarce labeled support data and limits task adaptation, which is the primary objective in few-shot learning. In this setting, conformal prediction should serve as an uncertainty estimation layer that supports the adapted model, rather than preventing adaptation itself. To this end, we propose AlignCP, a framework that reconciles supervised few-shot adaptation with conformal uncertainty estimation under non-exchangeability. AlignCP learns a reweighted calibration distribution that reduces the score-level discrepancy between the labeled support set and the unlabeled query set. By aligning the one-dimensional nonconformity score distributions, AlignCP aims to close the coverage gap induced by adaptation without requiring query labels.

==> table/comparison.tex <==
% \begin{table*}[t]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2.6pt}
% \renewcommand{\arraystretch}{1.12}
% \caption{\textbf{Conceptual comparison in few-shot medical-VLM conformal transfer.}
% ``Support fit'' means that labeled support examples update the task predictor; ``single model'' means that inference avoids candidate-label-specific refitting.
% Among the compared methods, \method explicitly studies the combination of supervised support fitting, one retained predictor, unlabeled-query calibration, and post-adaptation score repair. Its current coverage claim is empirical rather than the standard finite-sample SCP guarantee.}
% \label{tab:conceptual}
% \begin{tabularx}{\textwidth}{@{}lccc>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X@{}}
% \toprule
% \textbf{Method} & \textbf{Support fit} & \textbf{Query use} & \textbf{Single model} & \textbf{Handling of support-reuse mismatch} & \textbf{Coverage statement} & \textbf{Main limitation} \\
% \midrule
% SCP & No & No & Yes & Assumes the mismatch is absent. & Finite-sample under exchangeability. & No supervised task adaptation. \\
% Weighted CP \cite{tibshirani2019conformal} & No & Optional & Yes & Corrects specified covariate shift, not support reuse. & Finite-sample with correct shift weights. & Requires a correct or accurately estimated shift model. \\
% SemiCP \cite{zhou2026semi} & No & Yes & Yes & Augments scarce calibration using estimated unlabeled scores. & Asymptotic under its assumptions. & Fixed predictor; pseudo-score assumptions. \\
% NECP-OT \cite{correia2026non} & Not studied & Yes & Yes & Aligns scores to an unlabeled target-score envelope under generic shift. & Coverage-loss estimation / gap control. & Supervised support reuse is not its target setting. \\
% SCA-T / LATA \cite{silva2025trustworthy,bozorgtabar2026lata} & No & Yes & Yes & Avoids the mismatch through label-free transductive refinement. & SCP-style validity under stated assumptions. & Support labels are not used to fit the task predictor. \\
% FCA \cite{silva2025full} & Yes & Per query & No & Restores conformal symmetry by query- and label-specific fitting. & Finite-sample full-conformal validity. & Repeated inference-time model fitting. \\
% Adapt+SCP & Yes & No & Yes & No explicit correction after fitting. & No standard post-fit guarantee. & Frequently under-covers. \\
% \textbf{ALIGNCP} & \textbf{Yes} & \textbf{Yes} & \textbf{Yes} & \textbf{Reweights post-fit support scores toward the unlabeled query-score envelope.} & \textbf{Empirical target-coverage recovery.} & \textbf{No standard finite-sample SCP guarantee.} \\
% \bottomrule
% \end{tabularx}
% \end{table*}

==> table/conceptual.tex <==
\input{table/comparison}

\begin{table}[t]
\centering
\caption{Conceptual comparison of conformal prediction methods for medical VLM adaptation.}
\label{tab:conceptual_comparison}
\resizebox{\columnwidth}{!}{
\setlength{\tabcolsep}{15pt}
\begin{tabular}{lccc}
\toprule
\textbf{Method} 
& \textbf{Label Usage}
& \makecell{\textbf{Adaptation} \\ \textbf{Ability}}
& \makecell{\textbf{Empirical} \\ \textbf{Coverage}} \\
\midrule

SCP
& None
& Low
& \cmark \\

SCA-T
& Unlabeled
& Medium
& \cmark \\

Adapt + SCP
& Labeled
& High
& \xmark \\

\textbf{\ours{} (ours)}
& Labeled
& High
& \cmark \\

\bottomrule
\end{tabular}}
\end{table}




% \begin{table}[t]
% \centering
% % \caption{Conceptual comparison of conformal prediction methods under adaptation.}
% \caption{Conceptual comparison of conformal prediction methods for medical VLM adaptation.}
% \label{tab:conceptual_comparison}
% \resizebox{\columnwidth}{!}{
% \setlength{\tabcolsep}{15pt}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Method} 
% & \textbf{Training} 
% & \makecell{\textbf{Adaptation} \\ \textbf{Ability}}
% & \makecell{\textbf{Empirical} \\ \textbf{Coverage}} \\
% \midrule

% SCP
% & None
% & Low
% & \cmark \\

% SCAT \cite{silva2025trustworthy}
% & Unsupervised
% & Medium
% & \cmark \\

% Adapt + SCP \cite{silva2025trustworthy}
% & Supervised
% & High
% & \xmark \\

% \textbf{\ours{} (ours)}
% & Supervised
% & High
% & \cmark \\

% \bottomrule
% \end{tabular}}
% \end{table}



% \begin{table}[t]
% \centering
% \caption{Conceptual comparison of conformal prediction methods under adaptation.}
% \label{tab:conceptual_comparison}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Method} 
% & \textbf{Training} 
% & \textbf{Label Usage}
% & \makecell{\textbf{Adaptation} \\ \textbf{Ability}}
% & \makecell{\textbf{Adaptation-Shift} \\ \textbf{Correction}} \\
% \midrule
% SCP
% & None
% & None
% & Low
% & \xmark \\

% SCAT
% & Unsupervised
% & Unlabeled
% & Medium
% & \xmark \\

% Adapt + SCP
% & Supervised
% & Labeled
% & High
% & \xmark \\

% \textbf{\ours{} (ours)}
% & {Supervised}
% & {Labeled}
% & {High}
% & {\cmark} \\
% \bottomrule
% \end{tabular}}
% \end{table}
